Human-to-Human Interaction Detection

A comprehensive understanding of interested human-to-human interactions in video streams, such as queuing, handshaking, fighting and chasing, is of immense importance to the surveillance of public security in regions like campuses, squares and parks. Different from conventional human interaction recognition, which uses choreographed videos as inputs, neglects concurrent interactive groups, and performs detection and recognition in separate stages, we introduce a new task named human-to-human interaction detection (HID). HID devotes to detecting subjects, recognizing person-wise actions, and grouping people according to their interactive relations, in one model. First, based on the popular AVA dataset created for action detection, we establish a new HID benchmark, termed AVA-Interaction (AVA-I), by adding annotations on interactive relations in a frame-by-frame manner. AVA-I consists of 85,254 frames and 86,338 interactive groups, and each image includes up to 4 concurrent interactive groups. Second, we present a novel baseline approach SaMFormer for HID, containing a visual feature extractor, a split stage which leverages a Transformer-based model to decode action instances and interactive groups, and a merging stage which reconstructs the relationship between instances and groups. All SaMFormer components are jointly trained in an end-to-end manner. Extensive experiments on AVA-I validate the superiority of SaMFormer over representative methods. The dataset and code will be made public to encourage more follow-up studies.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> section/05_dataset.tex <==
\section{The AVA-Interaction Dataset}
\label{sec:avai}

% \begin{figure}[t!]
	%   \centering
	%   \includegraphics[width=0.48\textwidth]{figs/dataset_compare.pdf}
	%   \caption{The example of BIT (top-left), TVHI (top-right), UT (bottom-left) and AVA-Interaction (bottom-right).}
	%   \label{fig:dataset_compare}
	% \end{figure}

\begin{table}[htbp]
	\small
	\centering
	\begin{tabular}{l|cccc}
		& BIT    & UT    & TVHI  & AVA-I           \\
		\hline
		\# Interaction categories & 9      & 6     & 5     & \textbf{17}  \\
		Max \# group per frame   & 1      & 1     & 1     & \textbf{4}      \\
		Max \# people per group  & 2      & 2     & 2     & \textbf{13}     \\
		Mean \# people per group      & 2      & 2     & 2     & \textbf{2.5}    \\
		\# Annotated frames       & 12,896 & 9,228 & 2,815 & \textbf{85,254} \\
		\# Groups in total        & 12,896 & 9,228 & 2,815 & \textbf{8,6338}
	\end{tabular}%
	\caption{Compare the proposed AVA-I against existing datasets that are available to HID. AVA-I benchmarks HID \wrt. all aspects.}
	\label{tab:dataset_comparison}%
\end{table}%


\begin{figure}[t!]
	\centering
	\includegraphics[width=0.46\textwidth]{figs/data.pdf}
	\caption{The distribution of interactive classes in AVA-I.}
	\label{fig:label_statistic}
\end{figure}

As mentioned in Section~\ref{sec:related}, available datasets for HID fail to match practical human interactions in terms of scale and complexity. To fix this, we present a large-scale benchmark on HID in order to challenge the proposed SaMFormer and its baselines. Instead of building the benchmark from scratch, the proposed benchmark uses videos and annotations (including the bounding boxes and per-person interaction labels) from AVA \cite{ava}, which is a large-scale action detection dataset comprised of 437 YouTube videos and 80 atomic visual actions. For this reason, we name this new benchmark \emph{AVA-Interaction} (AVA-I).

To shape AVA (created for action detection) for HID, first we discard videos without any human-to-human interactions. Consequently, we obtain 298 videos containing 17 interactive action categories, see Figure~\ref{fig:label_statistic} for statistics. 
Since AVA does not cover interactive relations among people, we next annotate this information in a per-frame manner. To this end, we consider three scenarios for efficiency: 1) For frames that only include one person, they are simply discarded as any interaction must includes multiple participants; 2) For frames that exactly include two interactive people (the frame might take non-interactive people as well), the interactive relations are automatically recorded; 3) For all rest cases, human annotators are employed to carefully initialize the interactive relations, and the results are double-checked and corrected to improve the quality of annotation.

A comparison of AVA-I against existing datasets are shown in Table~\ref{tab:dataset_comparison}. AVA-I outperforms existing datasets in terms of numbers of annotated frames, total interactive groups, and interaction classes. AVA-I is also the best regarding the largest numbers of people and interactive groups per frame, as well as the average number of people per group. Unlike BIT and UT (acted and captured by amateurish actors and videographers), AVA-I interactions are highly realistic, thanks to the high-quality AVI videos sourced from TV-episodes. Our experiments are based on AVA-I unless otherwise stated.




